Interact with me: Joint Egocentric Forecasting of Intent to Interact, Attitude and Social Actions

For efficient human-agent interaction, an agent should proactively recognize their target user and prepare for upcoming interactions. We formulate this challenging problem as the novel task of jointly forecasting a person's intent to interact with the agent, their attitude towards the agent and the action they will perform, from the agent's (egocentric) perspective. So we propose \emph{SocialEgoNet} - a graph-based spatiotemporal framework that exploits task dependencies through a hierarchical multitask learning approach. SocialEgoNet uses whole-body skeletons (keypoints from face, hands and body) extracted from only 1 second of video input for high inference speed. For evaluation, we augment an existing egocentric human-agent interaction dataset with new class labels and bounding box annotations. Extensive experiments on this augmented dataset, named JPL-Social, demonstrate \emph{real-time} inference and superior performance (average accuracy across all tasks: 83.15\%) of our model outperforming several competitive baselines. The additional annotations and code will be available upon acceptance.

==> 5_experiments/4_temporal_modules.tex <==
\subsection{Effects of Different Temporal Modules}
\vspace{-1mm}
%
Table \ref{tab:temporal_module} studies the performance of various temporal modeling techniques within the SocialEgoNet.
%
Bi-LSTM consistently achieves the best results across all tasks with the best average F1 score (85.86\%), balancing performance and computational efficiency.
%
The transformer, also widely used in modeling sequential data, achieves comparable result to the Bi-LSTM for action prediction but is outperformed by 1D CNN for intent and attitude prediction tasks. This can be attributed to the smaller size of our dataset that favours smaller models.
%
The GCN, though has the fewest parameters and highest latency, does not perform as well as the others. 


==> 5_experiments/6_confusion.tex <==
\subsection{Confusion among Actions}
%
\vspace{-1mm}
Fig.~\ref{fig:cm} shows a confusion matrix for the action prediction task using results of SocialEgoNet. We observe that the difficulty in distinguishing between \texttt{pet} and \texttt{hug} while anticipating actions. This is due to similar movements observed from the \emph{ego view}, as in both cases the interacting subject raise their arm and reach toward the social agent to complete these actions. Two more actions, \texttt{point-converse} and \texttt{gaze}, are also confused often. This is expected since when humans point at the agent/robot and talk about it, they usually also look at it. Resolving this challenge may require information from additional modalities, such as audio.

==> 5_experiments/7_generalisation.tex <==
\subsection{Generalisation Capability}
Since the pose features are concise and the three downstream tasks are coupled to each other, it is possible that the framework overfitted and failed to learn generalisable social intelligence. Therefore, we mask a few samples of specific social actions during training and use them as a test set to test the generalisation ability of the proposed framework. Naturally, the framework cannot predict the classes of these unseen social actions. But if the framework can predict their social interests and attitudes, it confirms that the framework learns generalisable knowledge. We chose samples with hug, pet, punch, gaze, and leave masked during training and used them as the test set. There are masked samples for each social interest and attitude category. The framework consists of GCN+LSTM and the chain hierarchical classifier with an observation window of 30 frames. When predicting social interest, the framework has an F1 score of 0.71 and an accuracy of 72.29\%. When predicting social attitudes, the framework has an F1 score of 0.63 and an accuracy of 67.98\%. Even when analysing unseen user behaviours, the proposed framework still yields usable results with only one second of observation, which proves that the framework learns generalisable human social intelligence. 

==> figures/confusion.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.85\linewidth]{attachments/cm_action.png}
    \caption{The confusion matrix for action prediction using SocialEgoNet. Each element is normalized by its row sum so that diagonal entries represent the recall values. Most confused actions are: pet and hug; point and gaze.}
    \label{fig:cm}
\end{figure}

==> figures/confusion_matrices.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_interest_body.png}
    \caption{Social Intention Prediction Using Body}
    \label{fig:cm_action_body}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_interest_body_face.png}
    \caption{Social Intention Prediction Using Body and Face}
    \label{fig:cm_action_body_face}
\end{subfigure}
    \\
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_action_body.png}
    \caption{Social Action Prediction Using Body}
    \label{fig:cm_action_body}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_action_body_face.png}
    \caption{Social Action Prediction Using Body and Face}
    \label{fig:cm_action_body_face}
\end{subfigure}
    \\
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_action_body_hand.png}
    \caption{Social Action Prediction Using Body and Hands}
    \label{fig:cm_action_body_hand}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{attachments/cm_action.png}
    \caption{Social Action Prediction Using Whole-Body}
    \label{fig:cm_action}
\end{subfigure}
\caption{Confusion matrix for social actions prediction using different body parts. Comparing~\cref{fig:cm_action_body} and~\cref{fig:cm_action_body_face} shows that adding face keypoints allows SocialEgoNet to better discriminate if the user is interacting and social actions related to face area; comparing Figures~\cref{fig:cm_action_body} and~\cref{fig:cm_action_body_hand} shows that adding hand keypoints allows SocialEgoNet to better discriminate the social actions differently on the hands.}
\label{fig:cm}
\end{figure}

==> figures/data_distribution.tex <==
% \begin{figure*}[t]
% \centering
% % \begin{subfigure}{0.4\linewidth}
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{attachments/data_sample.png}
% %     \caption{Data Examples}
% %     \label{fig:data_sample}
% % \end{subfigure}
% \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[height=5cm]{attachments/pie_interest.png}
%     \caption{Social Interest}
%     \label{fig:pie_interest}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[height=5cm]{attachments/pie_attitude.png}
%     \caption{Social Attitude}
%     \label{fig:pie_attitude}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[height=5cm]{attachments/pie_action.png}
%     \caption{Social Action}
%     \label{fig:pie_action}
% \end{subfigure}
% \caption{Examples and distribution of all the categories of social interests, attitudes and actions.\TG{2(a) is too small to see the different actions properly, can you make the figure bigger} \YM{I will make new pie plots later.}}
% \label{fig:data}
% \end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{attachments/pie_charts/class_distribution.png}
\caption{
Details of the \textbf{JPL-4PS} dataset: Class distribution corresponding to the three tasks: intent (in \textbf{bold}), attitude (in \textit{italic}) and actions (in regular). The number of samples in each class is indicated in the parentheses, and the newly introduced labels are \underline{underscored}.
%\TG{I think you need to underscore 'interacting', interested, not interested as new labels. and also the attitudes.}
}
\label{fig:data}
\end{figure}

==> figures/data_samples.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{attachments/data_sample.png}
    \caption{Data Examples}
    \label{fig:data_sample}
\end{figure}

==> figures/framework.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{attachments/framework.png}
  \caption{The proposed framework for social understanding. \TG{We can remove this one now, if we put the teaser image above the abstract} }
  \label{fig:framework}
\end{figure}

==> figures/gcn.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{attachments/gcn.png}
    \caption{Model structure of the Graph Convolutional Network.}
    \label{fig:gcn}
\end{figure}

==> figures/hierachical.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{attachments/parallel.png}
    \caption{Parallel}
    \label{fig:parallel}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{attachments/tree.png}
    \caption{Tree}
    \label{fig:tree}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{attachments/chain.png}
    \caption{Chain}
    \label{fig:chain}
\end{subfigure}
\caption{Hierarchical classifiers \TG{Merge Fig 4 and 5 and create a large figure. Happy to help with the figures}}
\label{fig:hierachical}
\end{figure}

==> figures/model_structure_0.tex <==
\begin{figure*}[th]
    \centering
    \includegraphics[width=\textwidth]{attachments/model_structure_0.png}
    \caption{The structure of our proposed SocialEgoNet. We first utilize AlphaPose to generate whole-body key points from the input video clip. The key points of the face, body, and hands are then fed into separate Graph Neural Networks (GCNs) to extract spatial representations, which are subsequently fused by concatenation and then passed through a multi-head self-attention module (MSA). The fused spatial representations from each frame are concatenated and the resulting sequence is fed into a bidirectional LSTM to model temporal relationships. Finally, the spatiotemporal feature output from the LSTM is passed to a hierarchical classifier to generate predictions for the three tasks.}
    \label{fig:model_structure}
\end{figure*}

==> figures/model_structure_1.tex <==
\begin{figure*}[th]
    \centering
    \includegraphics[width=\textwidth]{attachments/model_structure_1.png}
    \caption{The structure of our proposed SocialEgoNet. We first utilize AlphaPose to generate whole-body key points from the input video clip. The key points of the face, body, and hands are then fed into separate Graph Neural Networks (GCNs) to extract spatial representations, which are subsequently fused by concatenation and then passed through a multi-head self-attention module (MSA). The fused spatial representations from each frame are concatenated and the resulting sequence is fed into a bidirectional LSTM to model temporal relationships. Finally, the spatiotemporal feature output from the LSTM is passed to a hierarchical classifier to generate predictions for the three tasks.}
    \label{fig:model_structure}
\end{figure*}

==> figures/vis_keypoints.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{attachments/vis_keypoints.png}
    \caption{Visualization of whole-body keypoints generated by AlphaPose on our dataset. The input is an image from the JPL dataset, cropped using our annotated bounding box. The output keypoints include 68 points for the face, 23 points for the body, and 42 points for the hands.}
    \label{fig:vis_keypoints}
\end{figure}

==> tables/temporal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|ccc|c}
\toprule
\textbf{Method} &
\begin{tabular}[c]{@{}c@{}}\textbf{Params} \\ (M) $\downarrow$ \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Latency} \\ (($\Delta +$) ms) $\downarrow$ \end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Intent} \\ \textbf{F1} (\%)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Attitude}\\ \textbf{F1} (\%)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Action}\\ \textbf{F1} (\%)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{F1} (\%)\end{tabular} \\ \midrule
1D-CNN           & {\ul 2.73}    & 0.22          & {\ul 92.02}    & {\ul 90.34}    & 71.81          & {\ul 84.72}    \\
GCN              & \textbf{2.59} & 0.31          & 90.30          & 89.08          & 69.51          & 82.96          \\
Transformer      & 4.58          & {\ul 0.18}    & 90.90          & 90.08          & {\ul 72.10}    & 84.36          \\
\textbf{Bi-LSTM} & 3.18          & \textbf{0.18} & \textbf{92.65} & \textbf{91.61} & \textbf{73.33} & \textbf{85.86} \\ \bottomrule
\end{tabular}%
}
\caption{The effects of using different methods to model the temporal dependency in SocialEgoNet. The best results are highlighted
in \textbf{bold}, while the second-best results are \underline{underscored}.}
\label{tab:temporal_module}
\end{table}

==> tables/variants.tex <==
% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|cc|cc}
% \hline
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Temporal\\ Module\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Classifier}} & \multicolumn{2}{c|}{\textbf{Average}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Latency\\ (ms)\end{tabular}}} \\ \cline{2-6}
%                                                                                     & Parallel       & Tree       & Chain      & F1 (\%)              & Acc. (\%)             &                                                                                &                                                                                  \\ \hline
% Bi-LSTM                                                                             &\cmark          &            &            &                      &                       &                                                                                &                                                                                  \\
% Bi-LSTM                                                                             &                &\cmark      &            &                      &                       &                                                                                &                                                                                  \\
% Bi-LSTM                                                                             &                &            &\cmark      &                      &                       &                                                                                &                                                                                  \\
% 1D CNN                                                                              &                &            &\cmark      &                      &                       &                                                                                &                                                                                  \\
% GCN                                                                                 &                &            &\cmark      &                      &                       &                                                                                &                                                                                  \\
% Transformer                                                                         &                &            &\cmark      &                      &                       &                                                                                &                                                                                  \\ \hline
% \end{tabular}%
% }
% \caption{Comparison between different temporal modules and classifiers in SocialEgoNet. \YM{Consider using something similar to this table instead of Tab.~\ref{tab:hierarchical_classifiers}, since this table focuses on all potential variants of our model. Comparing the results in the top three row demonstrates that using the Chain prediction head gives the best results. And that's why we also use the Chain head for other temporal modules.}\TB{Can we use 1 column for classifier? So that we will have more space for presenting performance.}}
% \label{tab:variants}
% \end{table}

\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|cc}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Module\\ Combination\end{tabular}}} & \textbf{Intent}  & \textbf{Attitude} & \textbf{Action}  & \textbf{Paras} & \textbf{Latency} \\
                                                                                       & \textbf{F1 (\%)} & \textbf{F1 (\%)}  & \textbf{F1 (\%)} & \textbf{(M)}   & \textbf{(ms)}    \\ \hline
Bi-LSTM + Parallel                                                                     & 87.24            & 86.99             & 67.81            & 3.18           & 0.17             \\
Bi-LSTM + Tree                                                                         & 90.27            & 89.28             & 71.16            & 3.18           & 0.17             \\
\textbf{Bi-LSTM + Chain}                                                               & \textbf{92.65}   & \textbf{91.61}    & \textbf{73.33}   & \textbf{3.18}  & \textbf{0.18}    \\
1D-CNN + Chain                                                                         & 92.02            & 90.34             & 71.81            & 2.73           & 0.22             \\
GCN + Chain                                                                            & 90.30            & 89.08             & 69.51            & 2.59           & 0.31             \\
Transformer + Chain                                                                    & 90.90            & 90.08             & 72.10            & 4.58           & 0.18             \\ \hline
\end{tabular}%
}
\caption{Comparison between different temporal modules and classifiers combinations in SocialEgoNet.} 
\label{tab:variants}
\end{table}
